Component Substitution through Dynamic Reconfigurations

Component substitution has numerous practical applications and constitutes an active research topic. This paper proposes to enrich an existing component-based framework--a model with dynamic reconfigurations making the system evolve--with a new reconfiguration operation which "substitutes" components by other components, and to study its impact on sequences of dynamic reconfigurations. Firstly, we define substitutability constraints which ensure the component encapsulation while performing reconfigurations by component substitutions. Then, we integrate them into a substitutability-based simulation to take these substituting reconfigurations into account on sequences of dynamic reconfigurations. Thirdly, as this new relation being in general undecidable for infinite-state systems, we propose a semi-algorithm to check it on the fly. Finally, we report on experimentations using the B tools to show the feasibility of the developed approach, and to illustrate the paper's proposals on an example of the HTTP server.

==> eptcsdata.tex <==
\providecommand{\firstpage}{32}
\providecommand{\publicationstatus}{B. Buhnova, L. Happe, J. Kofro\v n (Eds.): Formal Engineering\\
Approaches to Software Components and Architectures 2014\\
EPTCS 147, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.147.3}{10.4204/EPTCS.147.3}}
\pdfoutput=1

